Unified Deployment-Aware Evaluation of Open Reasoning Language Models

Open reasoning language models are often compared under mixed sample sizes, partially standardized prompts, and accuracy-centered summaries, which makes practical model selection difficult to interpret. We present a unified evaluation of seven open reasoning language model configurations across four benchmarks: ARC-Challenge, GSM8K, MATH levels 1 to 3, and TruthfulQA MC1. We test zero-shot, chain-of-thought (CoT), and few-shot CoT prompting on the same 238-example subset for every model--dataset--strategy condition, yielding a complete 7 x 4 x 3 design with 84 conditions and 19,992 evaluated examples. Beyond accuracy, we report Wilson confidence intervals, latency, peak video random access memory (VRAM), weighted aggregate performance, Pareto-efficient operating points, prompt-sensitivity metrics, and compatibility diagnostics. Gemma-4-26B-A4B with zero-shot prompting achieves the highest weighted score at 0.794. Gemma-4-E4B remains close to the top across prompting settings while using substantially lower latency and memory, making it a strong practical operating point. Bootstrap and paired-permutation analyses show that the leading configurations are close enough that deployment tradeoffs remain important. We also find that prompting strategy changes model rankings rather than shifting all models uniformly. Benchmark-specific complementarity creates routing headroom, with an oracle task-aware selector reaching a weighted score of 0.825. Compatibility diagnostics show that some apparent failures, especially Phi-4-Reasoning on GSM8K, reflect robustness and interface-adherence problems under the shared evaluation pipeline. These results support a central claim: open-model evaluation should be framed as a deployment-aware, multi-objective operating-point problem rather than as a single-score leaderboard exercise.

==> paper_assets/tables/table_best_per_dataset.tex <==
\begin{table}
\caption{Best-performing configuration for each dataset under the unified protocol.}
\label{tab:best-per-dataset}
\begin{tabular}{lllrrr}
\toprule
Dataset & BestModel & BestStrategy & Accuracy & LatencySec & VRAMGB \\
\midrule
ARC-Challenge & Gemma-4-26B-A4B & Zero-shot & 0.945 & 3.433 & 48.067 \\
GSM8K & Qwen3-8B & Few-shot CoT & 0.819 & 6.674 & 15.256 \\
MATH L1-L3 & Gemma-4-E4B & Few-shot CoT & 0.693 & 8.278 & 14.895 \\
TruthfulQA MC1 & Phi-4-Reasoning & Few-shot CoT & 1.000 & 4.362 & 27.305 \\
\bottomrule
\end{tabular}
\end{table}


==> paper_assets/tables/table_full_condition_matrix.tex <==
\begin{longtable}{lllrrrrrr}
\caption{Per-condition results under the unified 238-example protocol.} \label{tab:full-condition-matrix} \\
\toprule
Dataset & Model & Strategy & N & Accuracy & CILow & CIHigh & LatencySec & VRAMGB \\
\midrule
\endfirsthead
\caption[]{Per-condition results under the unified 238-example protocol.} \\
\toprule
Dataset & Model & Strategy & N & Accuracy & CILow & CIHigh & LatencySec & VRAMGB \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
ARC-Challenge & Gemma-4-26B-A4B & CoT & 238 & 0.891 & 0.845 & 0.924 & 3.132 & 48.067 \\
ARC-Challenge & Gemma-4-E2B & CoT & 238 & 0.769 & 0.711 & 0.818 & 0.450 & 9.543 \\
ARC-Challenge & Gemma-4-E4B & CoT & 238 & 0.891 & 0.845 & 0.924 & 0.496 & 14.895 \\
ARC-Challenge & Phi-4-Mini-Reasoning & CoT & 238 & 0.269 & 0.217 & 0.329 & 4.119 & 7.145 \\
ARC-Challenge & Phi-4-Reasoning & CoT & 238 & 0.294 & 0.240 & 0.355 & 4.830 & 27.305 \\
ARC-Challenge & Qwen3-30B-A3B & CoT & 238 & 0.395 & 0.335 & 0.458 & 10.307 & 57.621 \\
ARC-Challenge & Qwen3-8B & CoT & 238 & 0.340 & 0.283 & 0.403 & 5.193 & 15.256 \\
ARC-Challenge & Gemma-4-26B-A4B & Few-shot CoT & 238 & 0.937 & 0.899 & 0.961 & 2.765 & 48.067 \\
ARC-Challenge & Gemma-4-E2B & Few-shot CoT & 238 & 0.727 & 0.667 & 0.780 & 4.485 & 9.543 \\
ARC-Challenge & Gemma-4-E4B & Few-shot CoT & 238 & 0.891 & 0.845 & 0.924 & 0.831 & 14.895 \\
ARC-Challenge & Phi-4-Mini-Reasoning & Few-shot CoT & 238 & 0.290 & 0.236 & 0.351 & 4.088 & 7.145 \\
ARC-Challenge & Phi-4-Reasoning & Few-shot CoT & 238 & 0.277 & 0.224 & 0.337 & 4.854 & 27.305 \\
ARC-Challenge & Qwen3-30B-A3B & Few-shot CoT & 238 & 0.487 & 0.425 & 0.551 & 9.651 & 57.621 \\
ARC-Challenge & Qwen3-8B & Few-shot CoT & 238 & 0.525 & 0.462 & 0.588 & 4.889 & 15.256 \\
ARC-Challenge & Gemma-4-26B-A4B & Zero-shot & 238 & 0.945 & 0.909 & 0.968 & 3.433 & 48.067 \\
ARC-Challenge & Gemma-4-E2B & Zero-shot & 238 & 0.769 & 0.711 & 0.818 & 1.379 & 9.543 \\
ARC-Challenge & Gemma-4-E4B & Zero-shot & 238 & 0.899 & 0.854 & 0.931 & 0.154 & 14.895 \\
ARC-Challenge & Phi-4-Mini-Reasoning & Zero-shot & 238 & 0.273 & 0.220 & 0.333 & 4.089 & 7.145 \\
ARC-Challenge & Phi-4-Reasoning & Zero-shot & 238 & 0.303 & 0.248 & 0.364 & 4.853 & 27.305 \\
ARC-Challenge & Qwen3-30B-A3B & Zero-shot & 238 & 0.416 & 0.355 & 0.479 & 9.605 & 57.621 \\
ARC-Challenge & Qwen3-8B & Zero-shot & 238 & 0.445 & 0.384 & 0.509 & 4.897 & 15.256 \\
GSM8K & Gemma-4-26B-A4B & CoT & 238 & 0.782 & 0.725 & 0.829 & 11.617 & 48.067 \\
GSM8K & Gemma-4-E2B & CoT & 238 & 0.685 & 0.623 & 0.741 & 5.015 & 9.543 \\
GSM8K & Gemma-4-E4B & CoT & 238 & 0.790 & 0.734 & 0.837 & 5.076 & 14.895 \\
GSM8K & Phi-4-Mini-Reasoning & CoT & 238 & 0.210 & 0.163 & 0.266 & 8.433 & 7.145 \\
GSM8K & Phi-4-Reasoning & CoT & 238 & 0.008 & 0.002 & 0.030 & 9.810 & 27.305 \\
GSM8K & Qwen3-30B-A3B & CoT & 238 & 0.756 & 0.698 & 0.806 & 14.415 & 57.621 \\
GSM8K & Qwen3-8B & CoT & 238 & 0.790 & 0.734 & 0.837 & 6.871 & 15.256 \\
GSM8K & Gemma-4-26B-A4B & Few-shot CoT & 238 & 0.681 & 0.619 & 0.737 & 14.346 & 48.067 \\
GSM8K & Gemma-4-E2B & Few-shot CoT & 238 & 0.710 & 0.649 & 0.764 & 4.515 & 9.543 \\
GSM8K & Gemma-4-E4B & Few-shot CoT & 238 & 0.752 & 0.694 & 0.803 & 5.405 & 14.895 \\
GSM8K & Phi-4-Mini-Reasoning & Few-shot CoT & 238 & 0.315 & 0.259 & 0.377 & 8.153 & 7.145 \\
GSM8K & Phi-4-Reasoning & Few-shot CoT & 238 & 0.021 & 0.009 & 0.048 & 9.660 & 27.305 \\
GSM8K & Qwen3-30B-A3B & Few-shot CoT & 238 & 0.807 & 0.752 & 0.852 & 14.740 & 57.621 \\
GSM8K & Qwen3-8B & Few-shot CoT & 238 & 0.819 & 0.765 & 0.863 & 6.674 & 15.256 \\
GSM8K & Gemma-4-26B-A4B & Zero-shot & 238 & 0.794 & 0.738 & 0.841 & 8.921 & 48.067 \\
GSM8K & Gemma-4-E2B & Zero-shot & 238 & 0.693 & 0.632 & 0.748 & 4.549 & 9.543 \\
GSM8K & Gemma-4-E4B & Zero-shot & 238 & 0.790 & 0.734 & 0.837 & 4.931 & 14.895 \\
GSM8K & Phi-4-Mini-Reasoning & Zero-shot & 238 & 0.181 & 0.137 & 0.235 & 8.328 & 7.145 \\
GSM8K & Phi-4-Reasoning & Zero-shot & 238 & 0.042 & 0.023 & 0.076 & 9.731 & 27.305 \\
GSM8K & Qwen3-30B-A3B & Zero-shot & 238 & 0.782 & 0.725 & 0.829 & 14.302 & 57.621 \\
GSM8K & Qwen3-8B & Zero-shot & 238 & 0.790 & 0.734 & 0.837 & 6.664 & 15.256 \\
MATH L1-L3 & Gemma-4-26B-A4B & CoT & 238 & 0.643 & 0.580 & 0.701 & 17.412 & 48.067 \\
MATH L1-L3 & Gemma-4-E2B & CoT & 238 & 0.580 & 0.516 & 0.641 & 10.964 & 9.543 \\
MATH L1-L3 & Gemma-4-E4B & CoT & 238 & 0.668 & 0.606 & 0.725 & 10.833 & 14.895 \\
MATH L1-L3 & Phi-4-Mini-Reasoning & CoT & 238 & 0.223 & 0.174 & 0.280 & 16.378 & 7.145 \\
MATH L1-L3 & Phi-4-Reasoning & CoT & 238 & 0.013 & 0.004 & 0.036 & 19.318 & 27.305 \\
MATH L1-L3 & Qwen3-30B-A3B & CoT & 238 & 0.576 & 0.512 & 0.637 & 26.157 & 57.621 \\
MATH L1-L3 & Qwen3-8B & CoT & 238 & 0.277 & 0.224 & 0.337 & 13.506 & 15.256 \\
MATH L1-L3 & Gemma-4-26B-A4B & Few-shot CoT & 238 & 0.571 & 0.508 & 0.633 & 23.528 & 48.067 \\
MATH L1-L3 & Gemma-4-E2B & Few-shot CoT & 238 & 0.689 & 0.628 & 0.744 & 8.969 & 9.543 \\
MATH L1-L3 & Gemma-4-E4B & Few-shot CoT & 238 & 0.693 & 0.632 & 0.748 & 8.278 & 14.895 \\
MATH L1-L3 & Phi-4-Mini-Reasoning & Few-shot CoT & 238 & 0.391 & 0.331 & 0.454 & 16.543 & 7.145 \\
MATH L1-L3 & Phi-4-Reasoning & Few-shot CoT & 238 & 0.029 & 0.014 & 0.059 & 19.389 & 27.305 \\
MATH L1-L3 & Qwen3-30B-A3B & Few-shot CoT & 238 & 0.613 & 0.550 & 0.673 & 24.786 & 57.621 \\
MATH L1-L3 & Qwen3-8B & Few-shot CoT & 238 & 0.639 & 0.576 & 0.697 & 11.515 & 15.256 \\
MATH L1-L3 & Gemma-4-26B-A4B & Zero-shot & 238 & 0.693 & 0.632 & 0.748 & 14.125 & 48.067 \\
MATH L1-L3 & Gemma-4-E2B & Zero-shot & 238 & 0.618 & 0.555 & 0.677 & 11.851 & 9.543 \\
MATH L1-L3 & Gemma-4-E4B & Zero-shot & 238 & 0.630 & 0.567 & 0.689 & 11.952 & 14.895 \\
MATH L1-L3 & Phi-4-Mini-Reasoning & Zero-shot & 238 & 0.252 & 0.201 & 0.311 & 16.289 & 7.145 \\
MATH L1-L3 & Phi-4-Reasoning & Zero-shot & 238 & 0.038 & 0.020 & 0.070 & 19.265 & 27.305 \\
MATH L1-L3 & Qwen3-30B-A3B & Zero-shot & 238 & 0.584 & 0.521 & 0.645 & 27.392 & 57.621 \\
MATH L1-L3 & Qwen3-8B & Zero-shot & 238 & 0.218 & 0.171 & 0.275 & 13.270 & 15.256 \\
TruthfulQA MC1 & Gemma-4-26B-A4B & CoT & 238 & 0.727 & 0.667 & 0.780 & 2.698 & 48.067 \\
TruthfulQA MC1 & Gemma-4-E2B & CoT & 238 & 0.563 & 0.500 & 0.625 & 1.273 & 9.543 \\
TruthfulQA MC1 & Gemma-4-E4B & CoT & 238 & 0.643 & 0.580 & 0.701 & 2.476 & 14.895 \\
TruthfulQA MC1 & Phi-4-Mini-Reasoning & CoT & 238 & 0.983 & 0.958 & 0.993 & 4.092 & 7.145 \\
TruthfulQA MC1 & Phi-4-Reasoning & CoT & 238 & 0.996 & 0.977 & 0.999 & 4.600 & 27.305 \\
TruthfulQA MC1 & Qwen3-30B-A3B & CoT & 238 & 0.987 & 0.964 & 0.996 & 9.961 & 57.621 \\
TruthfulQA MC1 & Qwen3-8B & CoT & 238 & 0.987 & 0.964 & 0.996 & 5.156 & 15.256 \\
TruthfulQA MC1 & Gemma-4-26B-A4B & Few-shot CoT & 238 & 0.786 & 0.729 & 0.833 & 1.681 & 48.067 \\
TruthfulQA MC1 & Gemma-4-E2B & Few-shot CoT & 238 & 0.517 & 0.454 & 0.580 & 6.020 & 9.543 \\
TruthfulQA MC1 & Gemma-4-E4B & Few-shot CoT & 238 & 0.739 & 0.680 & 0.791 & 0.195 & 14.895 \\
TruthfulQA MC1 & Phi-4-Mini-Reasoning & Few-shot CoT & 238 & 0.966 & 0.935 & 0.983 & 4.143 & 7.145 \\
TruthfulQA MC1 & Phi-4-Reasoning & Few-shot CoT & 238 & 1.000 & 0.984 & 1.000 & 4.362 & 27.305 \\
TruthfulQA MC1 & Qwen3-30B-A3B & Few-shot CoT & 238 & 0.966 & 0.935 & 0.983 & 9.625 & 57.621 \\
TruthfulQA MC1 & Qwen3-8B & Few-shot CoT & 238 & 0.979 & 0.952 & 0.991 & 5.021 & 15.256 \\
TruthfulQA MC1 & Gemma-4-26B-A4B & Zero-shot & 238 & 0.794 & 0.738 & 0.841 & 2.653 & 48.067 \\
TruthfulQA MC1 & Gemma-4-E2B & Zero-shot & 238 & 0.550 & 0.487 & 0.612 & 2.613 & 9.543 \\
TruthfulQA MC1 & Gemma-4-E4B & Zero-shot & 238 & 0.735 & 0.676 & 0.787 & 0.456 & 14.895 \\
TruthfulQA MC1 & Phi-4-Mini-Reasoning & Zero-shot & 238 & 0.945 & 0.909 & 0.968 & 4.129 & 7.145 \\
TruthfulQA MC1 & Phi-4-Reasoning & Zero-shot & 238 & 0.996 & 0.977 & 0.999 & 4.403 & 27.305 \\
TruthfulQA MC1 & Qwen3-30B-A3B & Zero-shot & 238 & 0.983 & 0.958 & 0.993 & 9.907 & 57.621 \\
TruthfulQA MC1 & Qwen3-8B & Zero-shot & 238 & 0.962 & 0.930 & 0.980 & 4.586 & 15.256 \\
\end{longtable}


==> paper_assets/tables/table_top10_deployment.tex <==
\begin{table}
\caption{Top 10 configurations by weighted score, with deployment-oriented summary metrics.}
\label{tab:top10-deployment}
\begin{tabular}{llrrrr}
\toprule
Model & Strategy & WeightedAcc & MeanLatencySec & MeanVRAMGB & AccPerSec \\
\midrule
Gemma-4-26B-A4B & Zero-shot & 0.794 & 7.283 & 48.067 & 0.109 \\
Gemma-4-E4B & Few-shot CoT & 0.761 & 3.677 & 14.895 & 0.207 \\
Gemma-4-E4B & CoT & 0.759 & 4.720 & 14.895 & 0.161 \\
Gemma-4-E4B & Zero-shot & 0.758 & 4.373 & 14.895 & 0.173 \\
Gemma-4-26B-A4B & CoT & 0.756 & 8.715 & 48.067 & 0.087 \\
Qwen3-8B & Few-shot CoT & 0.722 & 7.025 & 15.256 & 0.103 \\
Gemma-4-26B-A4B & Few-shot CoT & 0.710 & 10.580 & 48.067 & 0.067 \\
Qwen3-30B-A3B & Few-shot CoT & 0.701 & 14.701 & 57.621 & 0.048 \\
Gemma-4-E2B & Few-shot CoT & 0.688 & 5.997 & 9.543 & 0.115 \\
Gemma-4-E2B & Zero-shot & 0.671 & 5.098 & 9.543 & 0.132 \\
\bottomrule
\end{tabular}
\end{table}


==> paper_assets/tables/table_weighted_ranking.tex <==
\begin{table}
\caption{Unified weighted ranking across all model-strategy configurations.}
\label{tab:weighted-ranking}
\begin{tabular}{llrrrr}
\toprule
Model & Strategy & WeightedAcc & MeanLatencySec & MeanVRAMGB & MeanTokensPerSec \\
\midrule
Gemma-4-26B-A4B & Zero-shot & 0.794 & 7.283 & 48.067 & 20.570 \\
Gemma-4-E4B & Few-shot CoT & 0.761 & 3.677 & 14.895 & 25.850 \\
Gemma-4-E4B & CoT & 0.759 & 4.720 & 14.895 & 25.615 \\
Gemma-4-E4B & Zero-shot & 0.758 & 4.373 & 14.895 & 25.684 \\
Gemma-4-26B-A4B & CoT & 0.756 & 8.715 & 48.067 & 19.960 \\
Qwen3-8B & Few-shot CoT & 0.722 & 7.025 & 15.256 & 49.419 \\
Gemma-4-26B-A4B & Few-shot CoT & 0.710 & 10.580 & 48.067 & 19.598 \\
Qwen3-30B-A3B & Few-shot CoT & 0.701 & 14.701 & 57.621 & 25.127 \\
Gemma-4-E2B & Few-shot CoT & 0.688 & 5.997 & 9.543 & 31.747 \\
Gemma-4-E2B & Zero-shot & 0.671 & 5.098 & 9.543 & 31.648 \\
Qwen3-30B-A3B & Zero-shot & 0.669 & 15.301 & 57.621 & 25.342 \\
Gemma-4-E2B & CoT & 0.658 & 4.425 & 9.543 & 31.600 \\
Qwen3-30B-A3B & CoT & 0.653 & 15.210 & 57.621 & 25.308 \\
Qwen3-8B & Zero-shot & 0.567 & 7.354 & 15.256 & 49.125 \\
Qwen3-8B & CoT & 0.566 & 7.682 & 15.256 & 49.450 \\
Phi-4-Mini-Reasoning & Few-shot CoT & 0.398 & 8.232 & 7.145 & 62.282 \\
Phi-4-Mini-Reasoning & CoT & 0.303 & 8.255 & 7.145 & 61.992 \\
Phi-4-Mini-Reasoning & Zero-shot & 0.297 & 8.209 & 7.145 & 62.240 \\
Phi-4-Reasoning & Zero-shot & 0.188 & 9.563 & 27.305 & 53.517 \\
Phi-4-Reasoning & Few-shot CoT & 0.173 & 9.566 & 27.305 & 54.165 \\
Phi-4-Reasoning & CoT & 0.166 & 9.639 & 27.305 & 53.244 \\
\bottomrule
\end{tabular}
\end{table}

